An efficient method for the anisotropic diffusion equation in magnetic fields

We solve the anisotropic diffusion equation in 2D, where the dominant direction of diffusion is defined by a vector field which does not conform to a Cartesian grid. Our method uses operator splitting to separate the diffusion perpendicular and parallel to the vector field. The slow time scale is solved using a provably stable finite difference formulation in the perpendicular to the vector field, and an integral operator for the diffusion parallel to it. Energy estimates are shown to for the continuous and semi-discrete cases. Numerical experiments are performed showing convergence of the method, and examples is given to demonstrate the capabilities of the method.

==> CTAC 2022 Proceedings/definitions.tex <==
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage[linesnumbered,boxed]{algorithm2e}
\usepackage[margin=20mm]{geometry} %Reduce margin size
\usepackage{amssymb}
\usepackage{latexsym}
\usepackage{listings}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{amsmath}
\usepackage{mathtools}
\usepackage{thmtools}
\usepackage[linesnumbered]{algorithm2e}
% \usepackage{natbib}
\usepackage{biblatex}
\graphicspath{ {Figures/} } %Use images from file location
\usepackage{color}
\usepackage{standalone} %For including out-sourced code
\usepackage[table,x11names]{xcolor}
\usepackage{soul}
\usepackage{multirow}
\usepackage{multicol}			%For multicol environments
\usepackage{caption}			%USE THESE TWO FOR
\usepackage{subcaption}		%CAPTIONS AND SUBCAPTIONS
\usepackage[colorlinks]{hyperref}
\hypersetup{citecolor = {blue},pdfauthor=author}
% \usepackage{cleveref}
\usepackage{tikz}
\usepackage{pgfplots}
\usepackage{sectsty}			%style package for sections
\usepackage{physics}
\usepackage{array}
\usepackage{float}
\usepackage{forest}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{multicol}
\usepackage{todonotes}

\usetikzlibrary{shapes,arrows,arrows.meta,decorations.pathmorphing,decorations.markings,decorations.pathreplacing,patterns,shapes.geometric}
\pgfplotsset{compat=1.12}
% put your command and environment definitions here
\setcounter{secnumdepth}{3}

%%%% Declare things for cmds
\DeclareMathOperator{\proj}{proj}

%%%% Document Formatting
\setlength{\parindent}{0mm} %Removes paragraph indents
\setlength{\parskip}{1em} %Remove paragraph indents

%%%% Commands
\newcommand{\numberthis}{\refstepcounter{equation}\tag{\theequation}}
\newcommand{\I}{\mathrm{i}\mkern1mu}  %Imaginary number
\newcommand{\e}[1]{\hat{e}_{#1}}  %Unit vector
\newcommand{\be}[1]{\mathbf{b}_{#1}} %Magnetic unit vector
\newcommand{\Id}[1]{\text{I}_{#1}}  %Identity matrix
\newcommand{\Ln}[2]{\norm{#2}_{#1}} %Ln norm
\newcommand{\vecproj}[2]{\proj_{#1}({#2})}  %Vector projection
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
% \newcommand{\dt}[1]{\frac{\text{d} #1}{\text{d}t}}
\newcommand{\tayterm}[3]{\frac{#1^#3 #2^#3}{#3!}}
\newcommand{\mbf}[1]{\mathbf{#1}}
\newcommand{\mB}{\mathbf{B}}
\newcommand{\mA}{\mathbf{A}}
\newcommand{\mE}{\mathbf{E}}
\newcommand{\mH}{\text{H}}
\newcommand{\vv}{\mathbf{v}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\pp}{\mathbf{p}}
\renewcommand{\qq}{\mathbf{q}}
\newcommand{\evalat}[2]{\left. #1 \right|_{#2}}


\newcommand{\half}{\frac{1}{2}}


% TABLES
\newcolumntype{C}{>{$}c<{$}}



\newtheorem{theorem}{Theorem}[section]
\theoremstyle{definition}
\newtheorem{lemma}{Lemma}

\declaretheoremstyle[
  numbered=yes,
  numberlike=theorem,
  spaceabove=1em plus 0.75em minus 0.25em,
  spacebelow=1em plus 0.75em minus 0.25em,
  qed={}%qed={end definition},%{\rule{2pt}{1em}},
]{exmpstyle}
\declaretheorem[
  style=exmpstyle,
  title=Definition,
  refname={definition,definitions},
  Refname={Definition,Definitions}
]{defn}


\newcommand{\logLogSlopeTriangle}[5]
{
    % #1. Relative offset in x direction.
    % #2. Width in x direction, so xA-xB.
    % #3. Relative offset in y direction.
    % #4. Slope d(y)/d(log10(x)).
    % #5. Plot options.

    \pgfplotsextra
    {
        \pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
        \pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
        \pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
        \pgfkeysgetvalue{/pgfplots/ymax}{\ymax}

        % Calculate auxilliary quantities, in relative sense.
        \pgfmathsetmacro{\xArel}{#1}
        \pgfmathsetmacro{\yArel}{#3}
        \pgfmathsetmacro{\xBrel}{#1-#2}
        \pgfmathsetmacro{\yBrel}{\yArel}
        \pgfmathsetmacro{\xCrel}{\xArel}
        %\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.

        \pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
        \pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
        \pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
        \pgfmathsetmacro{\lnyC}{\lnyA+(-#4)*(\lnxA-\lnxB)}
        \pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)} % THE IMPROVED EXPRESSION WITHOUT 'DIMENSION TOO LARGE' ERROR.

        % Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
        \coordinate (A) at (rel axis cs:\xArel,\yArel);
        \coordinate (B) at (rel axis cs:\xBrel,\yBrel);
        \coordinate (C) at (rel axis cs:\xCrel,\yCrel);

        % Draw slope triangle.
        \draw[#5]   (A) node[pos=0.5,anchor=north] {1}
                    (B)-- 
                    (C) node[xshift=0.2,yshift=0.2,pos=0.6,above] {#4};
    }
}

